A Deep Moving-camera Background Model

In video analysis, background models have many applications such as background/foreground separation, change detection, anomaly detection, tracking, and more. However, while learning such a model in a video captured by a static camera is a fairly-solved task, in the case of a Moving-camera Background Model (MCBM), the success has been far more modest due to algorithmic and scalability challenges that arise due to the camera motion. Thus, existing MCBMs are limited in their scope and their supported camera-motion types. These hurdles also impeded the employment, in this unsupervised task, of end-to-end solutions based on deep learning (DL). Moreover, existing MCBMs usually model the background either on the domain of a typically-large panoramic image or in an online fashion. Unfortunately, the former creates several problems, including poor scalability, while the latter prevents the recognition and leveraging of cases where the camera revisits previously-seen parts of the scene. This paper proposes a new method, called DeepMCBM, that eliminates all the aforementioned issues and achieves state-of-the-art results. Concretely, first we identify the difficulties associated with joint alignment of video frames in general and in a DL setting in particular. Next, we propose a new strategy for joint alignment that lets us use a spatial transformer net with neither a regularization nor any form of specialized (and non-differentiable) initialization. Coupled with an autoencoder conditioned on unwarped robust central moments (obtained from the joint alignment), this yields an end-to-end regularization-free MCBM that supports a broad range of camera motions and scales gracefully. We demonstrate DeepMCBM's utility on a variety of videos, including ones beyond the scope of other methods. Our code is available at https://github.com/BGU-CS-VIL/DeepMCBM .

==> figures/fig_compar_results_copy.tex <==
% \begin{figure}[!t]
\begin{figure}[H]
\newcommand{\methods}{0.30}
\newcommand{\notaplicableh}{31.94}
\newcommand{\notaplicablew}{49.15}
\centering
\subcaptionbox{{Input}}[\methods\linewidth]
{
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/input/00000_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/input/00030_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/input/00054_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/input/00000_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/input/00040_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/input/00079_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/input/in000401_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/input/in000501_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/input/in000601_resize.jpg}
% \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/input/00000_resize.jpg}
% \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/input/00050_resize.jpg}
% \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/input/00079_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/input/in000742_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/input/in000824_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/input/in001009_resize.jpg}
}
\subcaptionbox{{Ours}}[\methods\linewidth]
{
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/Ours/frame000000_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/Ours/frame000030_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/Ours/frame000054_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/Ours/frame000000_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/Ours/frame000040_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/Ours/frame000079_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/Ours/frame000400_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/Ours/frame000500_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/Ours/frame000600_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/Ours/frame000000_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/Ours/frame000050_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/Ours/frame000079_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/Ours/frame000741_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/Ours/frame000823_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/Ours/frame001008_resize.jpg}
}
\subcaptionbox{{JA-POLS}}[\methods\linewidth]
{
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/JA-POLS/f_0_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/JA-POLS/f_30_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/JA-POLS/f_54_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/JA-POLS/f_0_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/JA-POLS/f_40_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/JA-POLS/f_79_resize.jpg}
% \framebox(\notaplicableh,\notaplicablew){ 
% % \rotatebox{-90}{Inapplicable}
%     \begin{minipage}{1.6cm}
%  N/A: \\ large zoom changes failed\newline JA-POLS completely
% \end{minipage}
% }
    % \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/JA-POLS/f_400_resize.jpg}
    % \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/JA-POLS/f_500_resize.jpg}
    % \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/JA-POLS/f_600_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/JA-POLS/f_0_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/JA-POLS/f_50_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/JA-POLS/f_79_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/JA-POLS/f_141_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/JA-POLS/f_223_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/JA-POLS/f_408_resize.jpg}
}
\subcaptionbox{{PRPCA}}[\methods\linewidth]
{
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PRPCA/f_0_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PRPCA/f_30_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PRPCA/f_54_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PRPCA/f_0_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PRPCA/f_40_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PRPCA/f_79_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PRPCA/f_400_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PRPCA/f_500_resize.jpg}
    \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PRPCA/f_600_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PRPCA/f_0_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PRPCA/f_50_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PRPCA/f_79_resize.jpg}
%     \framebox(\notaplicableh,\notaplicablew){  
% %     \rotatebox{-90}{Inapplicable}
%     \begin{minipage}{1.5cm}
%  N/A: \\ out-of-memory \newline on a 256GB RAM machine
% \end{minipage}
%     }

}
\subcaptionbox{{PanGAEA}}[\methods\linewidth]
{
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PanGAEA/f_0000_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PanGAEA/f_0030_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PanGAEA/f_0054_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PanGAEA/f_0000_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PanGAEA/f_0040_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PanGAEA/f_0079_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PanGAEA/f_0400_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PanGAEA/f_0500_resize.jpg}
\includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PanGAEA/f_0600_resize.jpg}
% \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PanGAEA/f_0000_resize.jpg}
% \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PanGAEA/f_0050_resize.jpg}
% \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PanGAEA/f_0079_resize.jpg}
% \framebox(\notaplicableh,\notaplicablew){  
%     %     \rotatebox{-90}{Inapplicable}
%         \begin{minipage}{1.5cm}
%      N/A: \\ failed to run: Matlab process was killed
%     \end{minipage}
%         }
% \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/PanGAEA/f_0741_resize.jpg}
% \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/PanGAEA/f_0823_resize.jpg}
% \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/PanGAEA/f_1008_resize.jpg}
}
% \subcaptionbox{{PRAC}}[\methods\linewidth]
% {
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PRAC/f_0_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PRAC/f_30_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PRAC/f_54_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PRAC/f_0_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PRAC/f_40_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PRAC/f_79_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PRAC/f_400_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PRAC/f_500_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PRAC/f_600_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PRAC/f_0_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PRAC/f_50_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PRAC/f_79_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/PRAC/f_741_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/PRAC/f_823_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/PRAC/f_1008_resize.jpg}
% }
% \subcaptionbox{{PCP PTI}}[\methods\linewidth]
% {
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PCP_PTI/f_0_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PCP_PTI/f_30_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/dog-gooses/PCP_PTI/f_54_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PCP_PTI/f_0_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PCP_PTI/f_40_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/flamingo/PCP_PTI/f_79_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PCP_PTI/f_400_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PCP_PTI/f_500_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/zoomInZoomOut/PCP_PTI/f_600_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PCP_PTI/f_0_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PCP_PTI/f_50_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/bmx-trees/PCP_PTI/f_79_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/PCP_PTI/f_741_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/PCP_PTI/f_823_resize.jpg}
%     \includegraphics[width=\methods\linewidth,trim={0mm 0mm 0mm 0mm},clip]{./fig_compare_results_imgs/continuousPan/PCP_PTI/f_1008_resize.jpg}
% }
\\
\captionsetup{justification=raggedright, singlelinecheck=false}
\caption{Visual Comparison: Select Results. Note the ghosting artifacts
and/or distortion in the other methods' results. \textbf{Please zoom in to better appreciate the results.}}
\label{Fig:ResultsVisualComparison}

\end{figure}


==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\RD}{\ensuremath{\RR^D}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}




\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}
\newcommand{\WHITE}[1]{{{\color{white}{#1}}}}  

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{green}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  
\newcommand{\PURPLE}[1]{{{\color{purple}{#1}}}}  


\definecolor{brown}{RGB}{165,42,42}
\newcommand{\BROWN}[1]{{{\color{brown}{#1}}}}



\newcommand{\FREIFELD}[1]{\textbf{\MAGENTA{[FREIFELD says: #1]}}}
\newcommand{\MEITAR}[1]{\textbf{\BLUE{[MEITAR says: #1]}}}
\newcommand{\SHAHF}[1]{\textbf{\GREEN{[SHAHAF says: #1]}}}
% Make your own

\newcommand{\TBD}{\RED{[TBD]}}
\newcommand{\TODO}[1]{\RED{[TODO: #1]}}
\newcommand{\REPLACE}[2]{\RED{REPLACE:} \BLUE{#1} \RED{WITH:} \BLUE{#2}}


\newcommand{\SEtwo}{\ensuremath{\mathrm{SE}(2)}}


% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}
\bmdefine\bepsilon{\epsilon}


\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bsigma{\sigma}
\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbbm{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


 \newcommand{\DP}{\mathrm{DP}}
 \newcommand{\DIR}{\mathrm{Dir}}
 \newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


==> supmat/cpab.tex <==

\section{Diffeomorphisms}

Following recent incorporations of diffeomorphisms in STNs~\cite{Skafte:CVPR:2018:DDTN,Balakrishnan:CVPR:2018:unsupervised,Dalca:NIPS:2019:learning},
 we also evaluate the benefits of applying diffeomorphic-STN for MCBM. 
 
 \begin{definition}
  A ($C^1$) diffeomorphism is a differentiable invertible map with a differentiable inverse. 
 \end{definition}

 The advantages these qualities (a differentiable invertible map with a differentiable inverse) had been shown to increase expressiveness
 in the produced warps while maintaining stability during the training phase of DL models~\cite{Skafte:CVPR:2018:DDTN}.
In practice, however, incorporating diffeomorphisms usually involves expensive computations which might hinder their use in DL-frameworks.
The reason is that during training, evaluations
of $x\mapsto T^\btheta(x)$ (forward pass) and $x\mapsto \nabla_\btheta T^\btheta( x)$ (backward pass)
are computed at multiple points $x$ and for multiple $\btheta$'s. 
To mitigate this effect, while still maintaining expressiveness, we decide to follow~\cite{Skafte:CVPR:2018:DDTN} and incorporate 
CPAB warps, which were recently proposed in~\cite{Freifeld:ICCV:2015:CPAB,Freifeld:PAMI:2017:CPAB}. 
These warps had shown to combine expressiveness and efficiency in DL context~\cite{Hauberg:AISTATS:2016:DA,Skafte:CVPR:2018:DDTN}. 
Additionally, diffeomorphic temporal transformer networks were shown to be effective in the joint-alignment 
of time-series data~\cite{Kaufman:ICIP:2021:cyclic,Lohit:CVPR:2019:temporal,Shapira:NIPS:2019:DTAN}.
Thus, we also utilize the diffeomorphic STN for the task of jointly-aligning frames when building the panorama for our MCBM.
%
Below we briefly explain CPAB warps and refer the reader to~\cite{Freifeld:ICCV:2015:CPAB,Freifeld:PAMI:2017:CPAB,Freifeld:TR_CPAB_Derivaitive:2017}
for more details. 

\RED{Ron: did not change the part below}

\textbf{CPAB transformations:} transformations which are Based on Piecewise-Affine (CPA-Based) velocity fields.
The term ``piecewise'' is \wrt some partition, denoted by $\Omega$, of the input's domain into sub-intervals.
Let $\Vcal$ denote the linear space of CPA velocity fields \wrt such a fixed $\Omega$,
let $d=\dim(\Vcal)$, and let $v^\btheta:\Omega\to\RR$, a velocity field parametrized
by $\btheta\in\Rd$, denote the generic element
of $\Vcal$, where $\btheta$ stands for the coefficient \wrt some basis of $\Vcal$.
%
The corresponding space of CPAB warps, obtained via integration of elements of $\Vcal$,  is 
\begin{align}
 \Tcal\triangleq&
 %\set
 \{T^\btheta:
   x\mapsto \phi^\btheta( x;1)
  \text{ s.t. } \phi^\btheta( x;t) \text{ solves }  \\
  %\phi^\btheta(x;t)
  =& x+\int_{0}^t  v^\btheta(\phi^\btheta(x;\tau))\, 
 \mathrm{d}\tau \text{ where }  v^\btheta\in \Vcal\, \};
 \label{Eqn:IntegralEquation}
\end{align}
it can be shown that these warps are indeed ($C^1$) diffeomorphisms~\cite{Freifeld:ICCV:2015:CPAB,Freifeld:PAMI:2017:CPAB}.
While $v^\btheta$
is CPA, $T^\btheta:\Omega\to\Omega$ is not (\eg, $T^\btheta$ is differentiable).
% Also note that $T^\btheta$ is not piecewise-quadratic: $v^\btheta$ is
% integrated as a velocity field, not as a function.
CPA velocity fields support an
integration method that is faster \emph{and} more accurate than typical 
velocity-field integration methods~\cite{Freifeld:ICCV:2015:CPAB,Freifeld:PAMI:2017:CPAB}.
The fineness of  $\Omega$ controls the trade-off between expressiveness of $\Tcal$
on the one hand and the associated computational complexity and dimensionality on the other 
hand. 
%
%
%

% \textbf{Initialization.} Since $\btheta = \bzero$ gives the identity map 
% we initialize the CPAB layer by setting all the weights in the 
% final layer of the localization net to zero.

% \textbf{Optional zero-boundary conditions}. If of interest, one can easily restrict 
% the CPA fields to vanish at the endpoints of the domain, implying these points will be fixed points
% of of the resulting warp. 
% Importantly in the TTN context, the \emph{CPAB gradient},
% $\nabla_\btheta T^\btheta( x)$, is given by the efficient solution of
% a system of coupled integral 
% equations~\cite{Freifeld:PAMI:2017:CPAB}; see~\cite{Freifeld:TR_CPAB_Derivaitive:2017}
%  for details.








==> supmat/prelims.tex <==
\section{Spatial Transformer Networks} 
The Spatial Transformer Network (STN) \cite{Jaderberg:NIPS:2015:spatial} is a differentiable module that applies
 a parametrized spatial transformation in an input--dependent manner. 
Given a family of spatial transformations (\ie Affine) parametrized by $\btheta$ and an input image $U$, 
the STN predicts $\btheta$ and warps its input to produce $\mathcal{T}^{\btheta}(U)=V$ that minimize the loss of the downstream task.
The basic building blocks of the STN are as follows:
\begin{enumerate}
%
 \item \textbf{Localization network:} the localization network, $f_{\mathrm{loc}}$, is function which maps an input feature map $U$ to transformation 
 parameters $\btheta$, such that $f_{\mathrm{loc}}(\textbf{\textit{U}})=\btheta$. In the context of DL, $f_{\mathrm{loc}}$ is usually a regression
 neural network tasked to predict $\btheta$ by setting it's final layer to be $d=\dim(\btheta)$.
 %
 \item \textbf{Parameterised Sampling Grid:} a sampling grid $G \subset[-1,1] \times$ $[-1,1]$ of evenly-spaced points corresponding 
 to the width and height ($xy$) of the input. $G$ is transformed by the transformation $T^{\btheta}$ and is later used to interpolate pixel-values from the input $U$.

 %
 \item \textbf{Differentiable Image Sampling}. given $U, \btheta, \mathcal{T}$ and $G$, the sampler produce the output feature map $V$.
 A sampling kernel is applied to $U$ at $T^{\btheta}(G)$ to get the corresponding pixel value for the output $V$. 
 In practice, the inverse transformation is applied, $(T^{\btheta})^{-1}$, as specified in~\cite{Jaderberg:NIPS:2015:spatial}. 
 A popular choice is a bilinear sampling kernel.

\end{enumerate}


==> theorems.tex <==
\theoremstyle{definition}  
% \theoremsymbol{\scalebox{1}[1.4]{\large$ \diamond $}}
\newtheorem{Definition}{Definition}
\newtheorem{Example}{Example}
\newtheorem{Theorem}{Theorem}
\newtheorem*{Proof}{Proof}
\newtheorem{Remark}{Remark}

